An Improved Bayesian Semiparametric Model for Palaeoclimate Reconstruction: Cross-validation Based Model Assessment

Fossil-based palaeoclimate reconstruction is an important area of ecological science that has gained momentum in the backdrop of the global climate change debate. The hierarchical Bayesian paradigm provides an interesting platform for studying such important scientific issue. However, our cross-validation based assessment of the existing Bayesian hierarchical models with respect to two modern proxy data sets based on chironomid and pollen, respectively, revealed that the models are inadequate for the data sets. In this paper, we model the species assemblages (compositional data) by the zero-inflated multinomial distribution, while modelling the species response functions using Dirichlet process based Gaussian mixtures. This modelling strategy yielded significantly improved performances, and a formal Bayesian test of model adequacy, developed recently, showed that our new model is adequate for both the modern data sets. Furthermore, combining together the zero-inflated assumption, Importance Resampling Markov Chain Monte Carlo (IRMCMC) and the recently developed Transformation-based Markov Chain Monte Carlo (TMCMC), we develop a powerful and efficient computational methodology.

==> figures.tex <==

\begin{figure}
\includegraphics[width=7in,height=6.5in]{pics/scatterplots.pdf}
\caption{Pairwise scatterplots of the 4 variables used for clustering the Western Ghats data.
Different colours denote different clusters corresponding to the K-means clustering shown
in Figure \ref{fig:kmeans}.}
\label{fig:scatterplots}
\end{figure}

\begin{figure}
\includegraphics[width=7in,height=6.5in]{pics/wghats_kmeans_clustering.pdf}
\caption{$K$-means Clustering; different colours denote 11 different
clusters.
Cluster averages of mean (Mean) and standard deviation (SD) are shown in the legend.
}
\label{fig:kmeans}
\end{figure}


\begin{figure}
\includegraphics[width=7in,height=6.5in]{pics/wghats_clustering412.pdf}
\caption{Modal Central Clustering $C^{(412)}$; different colours denote 10 different
clusters.
Cluster averages of mean (Mean) and standard deviation (SD) are shown in the legend.
}
\label{fig:clustering412}
\end{figure}

\begin{figure}
\includegraphics[width=7in,height=6.5in]{pics/wghats_clustering759.pdf}
\caption{Modal Central Clustering $C^{(759)}$; different colours denote 14 different
clusters. 
Cluster averages of mean (Mean) and standard deviation (SD) are shown in the legend.
}
\label{fig:clustering759}
\end{figure}

\begin{figure}
\includegraphics[width=7in,height=6.5in]{pics/hpd_plots.pdf}
\caption{Plots of probabilities around each of the two modes $C^{(412)}$ and $C^{(759)}$ against the corresponding
HPD levels. These probabilities exclude the probabilities of the intersection of the two modal regions 
given by 
$Pr\left(\{C:\hat d(C^{(412)},C)<\epsilon_1\}\cap\{C:\hat d(C^{(759)},C)<\epsilon_2\}\right)$, the values of which are plotted
separately against the corresponding HPD levels for appropriate values of $\epsilon_1$ and $\epsilon_2$.}
\label{fig:hpd_sequence}
\end{figure}


\begin{figure}
\includegraphics[width=7in,height=6.5in]{pics/wghats_clustering_conditional.pdf}
\caption{Modal Conditional Central Clustering $C^{(1)}$; different colours denote 11 different
clusters.
The first component of each of the distinct mean values $\{\mu^*_{1j};j=1,\ldots,11\}$, associated with the clusters,
are shown in the legend.
}
\label{fig:clustering_conditional}
\end{figure}




==> tables.tex <==


\begin{table}
\caption{Two-way table showing number of observations in $C_i(I)\cap C_j(II),$ $i,j=1,\ldots,5$
for 5000 observations drawn from the normal mixture $\sum_{i=1}^5\frac{1}{5}N(i,1)$.
Clusterings $I$ and $II$ are obtained by $K$-means clustering with two different starting points.}
\label{table:table2}
\begin{center}
\begin{tabular}{|c|ccccc|c|}\hline
\multicolumn{1}{|c|}{\rule[-2mm]{0mm}{5mm}{Clusters of}}
& \multicolumn{5}{|c|}{\rule[-2mm]{0mm}{10mm}{Clusters of Clustering $II$}}
& \multicolumn{1}{|c|}{\rule[-2mm]{0mm}{5mm}}\\
Clustering $I$ & 1 & 2 & 3 & 4 & 5 & Row sum\\
\hline
1 & 0 & 0 & 0 & 60 & 639 & 699\\
2 & 0 & 229 & 1086 & 0 & 0 & 1315\\
3 & 639 & 0 & 0 & 0 & 0 & 639\\
4 & 0 & 0 & 143 & 1103 & 0 & 1246\\
5 & 166 & 935 & 0 & 0 & 0 & 1101\\
\hline
Col. sum & 805 & 1164 & 1229 & 1163 & 639 & 5000\\
\hline
\end{tabular}
\end{center}
\end{table}



\begin{table}
\caption{Two-way table showing number of units in $C_i(I)\cap C_j(II),$ $i,j=1,\ldots,11$
for the Western Ghats data. Row-wise clusters correspond to Clustering $I$
and column-wise clusters correspond to Clustering $II$.
Clusterings $I$ and $II$ are obtained by $K$-means clustering with two different starting points.}
\label{table:table3}
\begin{center}
\begin{tabular}{|c|ccccccccccc|c|}\hline
\multicolumn{1}{|c|}{\rule[-2mm]{0mm}{5mm}{Clusters of}}
& \multicolumn{11}{|c|}{\rule[-2mm]{0mm}{10mm}{Clusters of Clustering $II$}}
& \multicolumn{1}{|c|}{\rule[-2mm]{0mm}{5mm}}\\
Clustering $I$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & Row sum\\
\hline
1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2\\
2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 886 & 57 & 0 & 943\\
3 & 0 & 2 & 0 & 0 & 0 & 0 & 711 & 1432 & 1940 & 15 & 0 & 4100\\
4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 48 & 48\\
5 & 0 & 3 & 0 & 1781 & 0 & 0 & 86 & 0 & 2 & 0 & 0 & 1872\\
6 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 2\\
7 & 0 & 198 & 1076 & 86 & 77 & 0 & 6053 & 1877 & 0 & 0 & 0 & 9367\\
8 & 0 & 516 & 6859 & 4630 & 3683 & 0 & 2 & 0 & 0 & 0 & 0 & 15690\\
9 & 182 & 5 & 0 & 0 & 0 & 102 & 0 & 474 & 0 & 1920 & 0 & 2683\\
10 & 502 & 317 & 0 & 0 & 5686 & 10271 & 0 & 127 & 0 & 0 & 0 & 16903\\
11 & 214 & 2 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 7 & 224\\
\hline
Col. sum & 898 & 1043 & 7935 & 6498 & 9446 & 10373 & 6852 & 3910 & 2830 & 1992 & 57 & 51834\\
\hline
\end{tabular}
\end{center}
\end{table}



\begin{table}
\caption{Two-way table showing number of units in $C_i(I)\cap C_j(II),$ $i,j=1,\ldots,11$
for the Western Ghats data. Row-wise clusters correspond to Clustering $I$
with three variables and column-wise clusters correspond to Clustering $II$ with four variables.
Clusterings $I$ and $II$ are obtained by $K$-means clustering.}
\label{table:table4}
\begin{center}
\begin{tabular}{|c|ccccccccccc|c|}\hline
\multicolumn{1}{|c|}{\rule[-2mm]{0mm}{5mm}{Clusters of}}
& \multicolumn{11}{|c|}{\rule[-2mm]{0mm}{10mm}{Clusters of Clustering $II$}}
& \multicolumn{1}{|c|}{\rule[-2mm]{0mm}{5mm}}\\
Clustering $I$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & Row sum\\
\hline
1 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 2\\
2 & 0 & 929 & 158 & 0 & 2 & 0 & 0 & 0 & 1 & 0 & 0 & 1090\\
3 & 0 & 0 & 3814 & 0 & 6 & 0 & 252 & 0 & 0 & 0 & 0 & 4072\\
4 & 0 & 0 & 0 & 39 & 1796 & 0 & 78 & 1085 & 0 & 0 & 1 & 2999\\
5 & 0 & 0 & 0 & 0 & 23 & 0 & 8663 & 3 & 0 & 0 & 1 & 8690\\
6 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 197 & 4067 & 45 & 4309\\
7 & 0 & 0 & 0 & 0 & 41 & 0 & 44 & 9622 & 0 & 0 & 1 & 9708\\
8 & 0 & 14 & 128 & 0 & 0 & 0 & 49 & 0 & 2451 & 30 & 7 & 2679\\
9 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 9737 & 0 & 9738\\
10 & 2 & 0 & 0 & 9 & 0 & 0 & 0 & 0 & 33 & 13 & 156 & 213\\
11 & 0 & 0 & 0 & 0 & 4 & 0 & 281 & 4980 & 0 & 3056 & 13 & 8334\\
\hline
Col. sum & 2 & 943  & 4100 & 48 & 1872 & 2 & 9367 & 15690 & 2683 & 16903 & 224 & 51834\\
\hline
\end{tabular}
\end{center}
\end{table}




